Refinements of Futures Past: Higher-Order Specification with Implicit Refinement Types (Extended Version)

Refinement types decorate types with assertions that enable automatic verification. Like assertions, refinements are limited to binders that are in scope, and hence, cannot express higher-order specifications. Ghost variables circumvent this limitation but are prohibitively tedious to use as the programmer must divine and explicate their values at all call-sites. We introduce Implicit Refinement Types which turn ghost variables into implicit pair and function types, in a way that lets the refinement typechecker automatically synthesize their values at compile time. Implicit Refinement Types further take advantage of refinement type information, allowing them to be used as a lightweight verification tool, rather than merely as a technique to automate programming tasks. We evaluate the utility of Implicit Refinement Types by showing how they enable the modular specification and automatic verification of various higher-order examples including stateful protocols, access control, and resource usage.

==> 02-tick.tex <==

%\subsection{Resource Usage} \label{subsec:examples:tick}

%% Next, we show how to use Implicit Refinement Types to 
%% intrinsically verify resource usage. 
%% %
%% We show how to implement the applicative functor 
%% \ha{Tick} (\figref{fig:tick}) from \citet{liquidate} 
%% which is the identity functor annotated with a 
%% phantom parameter \ha{t} that tracks the resource 
%% usage (or ``cost'') of the underlying computation.
%% %
%% For brevity, we define a singleton form (\ha{T}).
%% 
%% \mypara{Counting Calls}
%% %
%% We \emph{count} resource usage by using our versions 
%% of two combinators from \citet{liquidate}:
%% %
%% First, \ha{pure} allows us to inject a value 
%% into the applicative context. 
%% %
%% \ha{pure} make no calls to functions whose 
%% call count is tracked by \ha{Tick}, so it 
%% safely asserts that the cost is $0$.
%% %
%% Second, \ha{</>} is a refined version of 
%% the standard applicative sequencing operator 
%% (typically written \ha{<*>}).
%% %
%% \ha{</>} takes two concrete arguments, 
%% a computation of a function and a computation 
%% of its argument, both wrapped in the \ha{Tick} context.
%% %
%% We then use Refinement Implicits to lift
%% the resource usage of both as the implicit
%% parameters \ha{n} and \ha{m}.
%% %
%% \ha{</>} is meant to be used for tracking 
%% resource usage: so we define the total 
%% resource usage of the combined computation 
%% (which applies the function to its argument) 
%% as \ha{n + m + 1}, adding the extra 1 to 
%% count the invocation of the sequencing combinator.
%% 
%% \mypara{Verifying append}
%% %
%% The type ascribed to \ha{(++)} specifies 
%% the \emph{resource usage} of \ha{(++)} 
%% and the length of the returned list. 
%% %
%% The signature says that \ha{(++)} 
%% takes two lists and produces a 
%% \ha{Tick} value whose cost equals 
%% the length of the first list 
%% and computes a list whose length 
%% equals the sum of the lengths of 
%% the input lists.
%% %
%% Let us focus on the novel specification 
%% on resource usage.
%% %
%% In the base case of \ha{++}, we simply use \ha{pure} to 
%% inject \ha{ys} into the applicative.
%% %
%% This computation then has cost $0$ which 
%% satisfies our obligation that 
%% append has cost equal to the 
%% length of the (empty) first list.
%% %
%% Both combinators are used in defining 
%% the recursive case of \ha{++}.
%% %
%% First, we inject a computation consing 
%% the head of the list into \ha{Tick} using 
%% \ha{pure} which has a cost of 0.
%% %
%% We then employ our \ha{</>} combinator 
%% to apply the consing to the recursive call, 
%% which by assumption, has cost \ha{len xs'}, 
%% so the cost of the overall computation is 
%% \ha{0 + len xs' + 1} which the SMT solver 
%% readily equates to the goal \ha{len xs}.
%% %
%% Thus, in both cases, we have verified 
%% that the cost  of \ha{++} equals 
%% the length of the first list \ha{xs}.
%% %
%% Again, the programmer did not 
%% have to supply the ghost parameters: 
%% our system inferred the instantiations 
%% from the two arguments of the \ha{</>} combinator.



==> 08-proofs.tex <==

\section{Appendix: Proofs}
\label{sec:proofs}

We include below the proofs of the key theorems.

Proof in \appref{sec:proofs} by induction on the satisfying contexts.

\begin{lemma}\label{alpha}
  $\poke{\h{c}[\h{R}/\h\kappa]} = \poke{\h{c}} [\h{R}/\h{\kappa}]$
\end{lemma}
Proof in \appref{sec:proofs} by induction on \h{c}.
\begin{lemma}\label{beta}
  $\Delta \vDash \poke{\h{c}\{\h{p}/\h{n}\}}$ iff
  $\Delta \vDash \poke{\h{c}} [\lambda\h{ n }.\h{ p = n}/\h{\pvar{n}}]$
\end{lemma}
Proof in \appref{sec:proofs} by induction on \h{c}.

\subsubsection{Side conditions}
\label{sec:decomposition}
Note that we can solve the \nosidesym{} and \sidesym{} cases separately:

\begin{theorem} \label{nosideside}
  $\valid{\h{\Delta}}{\h{\Psi}}{\noside{\poke{\h{c}}} \wedge \sides{\poke{\h c}}}$ iff $\valid{\h{\Delta}}{\h{\Psi}}{\poke{\h{c}}}$
\end{theorem}
\begin{lemma} \label{thm:nosidennf}
  $\noside{\poke{\h c}}$ is an \textsc{nnf} Horn Clause
\end{lemma}
\begin{proof}
  Each of these follow straightforwardly from induction on \h{c}
\end{proof}



\begin{proof} (Lemma~\ref{lem:strong})
%
Assume that $\pred \equiv \kvapp{\kvar}{z}$ where $\params{z} = \args{\kvar}$
The other cases are trivial as
$\apply{\ssoln{\cstr}{\kvar}}{\pred} = \pred$,
and
$\apply{\soln}{\pred_1} \Rightarrow \pred_1$ and
$\apply{\soln}{\pred_2} \Rightarrow \pred_2$
implies
$\apply{\soln}{\csand{\pred_1}{\pred_2}} \Rightarrow \csand{\pred_1}{\pred_2}$.
%
% \BLC{What if p = k(z) $\land$ r? ANS: prove the case for each conjunct separately and s(r1) => r1, s(r2) => r2 implies s(r1 /\ r2) => r1 /\ r2}
%
The proof is by induction on the structure of $\cstr$.
%
\begin{alignat}{3}
\intertext{\quad \emph{Case: $\cstr \equiv \kvapp{\kvar}{y}$.}}
\bcoz{By definition of $\solk{\cstr}{\kvar}$}
  && \apply{\ssoln{\cstr}{\kvar}}{\kvapp{\kvar}{z}} & = \params{z} = \params{y} \label{eq:zeqy}\\
\bcoz{Assume}
  && \soln, \binds{x_i}{\pred_i} & \models \kvapp{\kvar}{y} \notag \\
\bcoz{Hence}
  && \soln, \binds{x_i}{\pred_i} & \models \params{z} = \params{y} \Rightarrow \kvapp{\kvar}{z} \notag \\
\bcoz{By~\ref{eq:zeqy}}
  && \soln, \binds{x_i}{\pred_i} & \models \apply{\ssoln{\cstr}{\kvar}}{\kvapp{\kvar}{z}} \Rightarrow \kvapp{\kvar}{z} \notag \\
\intertext{\quad \emph{Case: $\cstr \equiv \pred'$, such that $\kvar \not \in \pred'$.}}
\bcoz{By definition of validity}
  && \soln, \binds{x_i}{\pred_i} & \models \tfalse \Rightarrow \kvapp{\kvar}{z} \notag \\
\bcoz{By the definition of $\solk{\cstr}{\kvar}$}
  && \apply{\ssoln{\cstr}{\kvar}}{\kvapp{\kvar}{z}} & = \tfalse \notag \\
\bcoz{Hence,}
  && \soln, \binds{x_i}{\pred_i} & \models \apply{ \ssoln{\cstr}{\kvar}   }{\kvapp{\kvar}{z}} \Rightarrow \kvapp{\kvar}{z} \notag \\
\intertext{\quad \emph{Case: $\cstr \equiv \csand{\cstr_1}{\cstr_2}$.}}
\intertext{\quad \quad Let $\pred_j = \solk{\cstr_j}{\kvar}$ for $j = 1,2$}
\bcoz{Thus, by the definition of $\solk{\cstr}{\kvar}$}
  &&\apply{\ssoln{\cstr}{\kvar}}{\kvapp{\kvar}{z}} & = \pred_1 \vee \pred_2 \label{eq:def-or} \\
\bcoz{Assume, for $j = 1,2$}
  && \soln, \binds{x_i}{\pred_i} & \models \wedge_j \cstr_j \notag \\
\bcoz{That is, for $j = 1,2$}
  && \soln, \binds{x_i}{\pred_i} & \models \cstr_j \notag \\
\bcoz{By IH, for $j = 1,2$}
  && \soln, \binds{x_i}{\pred_i} & \models \pred_j \Rightarrow \kvapp{\kvar}{z} \notag \\
\bcoz{Hence,}
  && \soln, \binds{x_i}{\pred_i} & \models (\pred_1 \vee \pred_2) \Rightarrow \kvapp{\kvar}{z} \notag \\
\bcoz{Thus, by~\ref{eq:def-or},}
  && \soln, \binds{x_i}{\pred_i} & \models \apply{\ssoln{\cstr}{\kvar}}{\kvapp{\kvar}{z}} \Rightarrow \kvapp{\kvar}{z} \notag \\
\intertext{\quad \emph{Case: $\cstr \equiv \csimp{x}{\base}{\pred}{\cstr'}$.}}
\intertext{\quad \quad Let $\pred' = \solk{\cstr'}{\kvar}$.}
\bcoz{Thus, by the definition of $\solk{\cstr}{\kvar}$}
  && \apply{\ssoln{\cstr'}{\kvar}}{\kvapp{\kvar}{z}} & = \pred'                                  \label{eq:def-imp-1} \\
  && \apply{\ssoln{\cstr}{\kvar}}{\kvapp{\kvar}{z}}  & = \existsp{x}{\base}{\pred \wedge \pred'} \label{eq:def-imp-2} \\
\bcoz{Assume}
  && \soln, \binds{x_i}{\pred_i} & \models \csimp{x}{\base}{\pred}{\cstr'} \notag \\
\bcoz{By \rulename{Sat-Ext}}
  && \soln, \binds{x_i}{\pred_i}, \bind{x}{\pred} & \models \cstr' \notag \\
\bcoz{By IH}
  && \soln, \binds{x_i}{\pred_i}, \bind{x}{\pred} & \models \apply{\ssoln{\cstr'}{\kvar}}{\kvapp{\kvar}{z}} \Rightarrow \kvapp{\kvar}{z} \notag \\
\bcoz{By~\ref{eq:def-imp-1}}
  && \soln, \binds{x_i}{\pred_i}, \bind{x}{\pred} & \models \pred' \Rightarrow \kvapp{\kvar}{z} \notag \\
\bcoz{By \rulename{Sat-Ext}}
  && \soln, \binds{x_i}{\pred_i} & \models \csimp{x}{\base}{\pred}{\pred' \Rightarrow \kvapp{\kvar}{z}} \notag \\
\bcoz{That is,}
  && \soln, \binds{x_i}{\pred_i} & \models \csimp{x}{\base}{(\pred \wedge \pred'}{\kvapp{\kvar}{z})} \notag \\
\bcoz{As $x \not \in \kvapp{\kvar}{z}$}
  && \soln, \binds{x_i}{\pred_i} & \models (\existsp{x}{\base}{\pred \wedge \pred'}) \Rightarrow \kvapp{\kvar}{z} \notag \\ %\mbox{\BLC{Can SAT-EXT be used like that? ANS: if x not in B, (ex x. A) => B EQUIV forall x.(A => B).}}\notag \\
\bcoz{By~\ref{eq:def-imp-2}}
  && \soln, \binds{x_i}{\pred_i} & \models  \apply{\ssoln{\cstr}{\kvar}}{\kvapp{\kvar}{z}} \Rightarrow \kvapp{\kvar}{z} \notag
\end{alignat}
\end{proof}

% forall x. (p(x) => q => r)

\begin{proof} (Theorem~\ref{lem:defns})
  The proof is an induction on the structure of $\cstr$.
  %
  \begin{alignat}{3}
  \intertext{\quad \emph{Case: $\cstr \equiv \kvapp{\kvar}{y}$.}}
    \bcoz{By definition}
    && \defns{\cstr}{\kvar}        & \doteq \kvapp{\kvar}{y} \notag \\
    \bcoz{and}
    && \ssoln{\cstr}{\kvar}(\kvar) & \doteq \lambda \params{x}. \wedge_i x_i = y_i \quad \mbox{ where } \params{x} = \args{\kvar} \notag \\
    \bcoz{Hence,}
    && \apply{\ssoln{\cstr}{\kvar}}{\defns{\cstr}{\kvar}}
                                   & \doteq \wedge_i y_i = y_i \label{eq:tauto1}\\
    \bcoz{As~\ref{eq:tauto1} is a tautology} %, \rulename{Sat-Base} yields}
    && \ssoln{\cstr}{\kvar}        & \models \defns{\cstr}{\kvar} \notag \\
%
  \intertext{\quad \emph{Case: $\cstr \equiv \pred$.}}
    \bcoz{By definition}
    && \defns{\cstr}{\kvar}        & \doteq \ttrue \notag \\
    \bcoz{Hence,}
    && \apply{\ssoln{\cstr}{\kvar}}{\defns{\cstr}{\kvar}}
                                   & \doteq \ttrue \label{eq:tauto2}\\
    \bcoz{As~\ref{eq:tauto2} is a tautology} %, \rulename{Sat-Base} yields}
    && \ssoln{\cstr}{\kvar}        & \models \defns{\cstr}{\kvar} \notag \\
%
\intertext{\quad \emph{Case: $\cstr \equiv \csand{\cstr_1}{\cstr_2}$.}}
\intertext{\quad \quad
  For $i \in \{ 1, 2\}$, let
    $\pred_i = \solk{\kvar}{\cstr_i}$,
    $\ssoln{\cstr_i}{\kvar}(\kvar) =  \lambda \params{x}. \pred_i$.
  }
%
  \bcoz{By definition}
    && \defns{\cstr}{\kvar}          & \doteq \defns{\cstr_1}{\kvar} \cup \defns{\cstr_2}{\kvar} \label{eq:union} \\
  \bcoz{By IH}
    && \ssoln{\cstr_i}{\kvar}                       & \models \defns{\cstr_i}{\kvar} \label{eq:ih-1} \\
  \intertext{\quad Let $\cstr' \in \defns{\cstr_i}{\kvar}$. As $\kvar$ \emph{only} in head,
   $\cstr' \equiv \csimpss{y}{\pred}{\kvapp{\kvar}{x}}$.}
  \bcoz{By \ref{eq:ih-1}}
    && \binds{y}{\pred} & \models \apply{\ssoln{\cstr_i}{\kvar}}{\kvapp{\kvar}{x}} \notag \\
  \bcoz{By Lemma~\ref{lem:weakening}}
    && \binds{y}{\pred} & \models \apply{\ssoln{\cstr_1}{\kvar}}{\kvapp{\kvar}{x}} \vee \apply{\ssoln{\cstr_2}{\kvar}}{\kvapp{\kvar}{x}} \notag \\
  \bcoz{That is}
    && \binds{y}{\pred} & \models \apply{\ssoln{\cstr}{\kvar}}{\kvapp{\kvar}{x}} \notag \\
  \bcoz{So for any $\cstr' \in \defns{\cstr_i}{\kvar}$}
    && \ssoln{\cstr}{\kvar} & \models \cstr' \notag \\
  \bcoz{Hence}
    && \ssoln{\cstr}{\kvar} & \models \defns{\cstr_i}{\kvar} \notag \\
  \bcoz{and hence, by~\ref{eq:union}}
    && \ssoln{\cstr}{\kvar} & \models \defns{\cstr}{\kvar} \notag \\
%
\intertext{\quad \emph{Case: $\cstr \equiv \csimp{x}{\base}{\pred}{\cstr'}$.}}
\intertext{\quad \quad
  Let $\pred' = \solk{\kvar}{\cstr'}$,
      $\soln' = \mapsingle{\kvar}{\lambda \params{z}. \pred'}$, and
      $\ssoln{\cstr}{\kvar} = \mapsingle{\kvar}{\lambda \params{z}. \existsp{x}{\base}{\pred \wedge \pred'}}$,
  }
%
  \bcoz{By IH}
    && \soln' & \models \defns{\cstr'}{\kvar} \label{eq:models-inner} \\
\intertext{\quad \quad Consider any arbitrary $\cstr'' \in \defns{\cstr'}{\kvar}$.}
  \bcoz{As $\kvar\in\head{\cstr''}$}
    && \cstr'' & \doteq \csimps{x_1}{\pred_1}{ \ldots \Rightarrow \csimps{x_n}{\pred_n}{\kvapp{\kvar}{y}}} \label{eq:inner-def}\\
  \bcoz{By~\ref{eq:models-inner}}
    && \soln'  & \models \csimps{x_1}{\pred_1}{ \ldots \Rightarrow \csimps{x_n}{\pred_n}{\kvapp{\kvar}{y}}} \notag \\
  \bcoz{By \rulename{Sat-Base}}
    && []      & \models \csimps{x_1}{\pred_1}{ \ldots \Rightarrow \csimps{x_n}{\pred_n}{ \subst{\pred'}{\params{z}}{\params{y}} }} \notag \\
  \bcoz{By \rulename{Sat-Ext}}
    && \binds{x_i}{\pred_i} & \models \subst{\pred'}{\params{z}}{\params{y}}  \label{eq:imp-a}\\
  \bcoz{Trivially,} % by definition of validity}
    && \bind{x}{\pred} & \models \pred \label{eq:imp-b}\\
  \bcoz{Hence, by~\ref{eq:imp-a},~\ref{eq:imp-b}} %and definition of validity}
    && \bind{x}{\pred}, \binds{x_i}{\pred_i} & \models {\pred \wedge \subst{\pred'}{\params{z}}{\params{y}}} \notag \\
  \bcoz{and so by definition of validity}
    && \bind{x}{\pred}, \binds{x_i}{\pred_i} & \models \existsp{x}{\base}{\pred \wedge \subst{\pred'}{\params{z}}{\params{y}}} \notag \\
  \bcoz{by~\ref{eq:inner-def}}
    && \ssoln{\cstr}{\kvar} & \models \csimp{x}{\base}{\pred}{\cstr''} \notag
\end{alignat}
  \quad \quad As the above holds for an arbitrary $\cstr'' \in \defns{\cstr'}{\kvar}$, we get $\satisfies{\ssoln{\cstr}{\kvar}}{\defns{\cstr}{\kvar}}$.
    % && \soln & \models \defns{\csimp{x}{\base}{\pred}{\cstr'}}{\kvar} \notag \\
\end{proof}

\begin{proof} (Theorem~\ref{thm:defns})
%
\vspace{-0.1in}
%
Let $\scoped{\kvar}{\cstr} \doteq \csimpss{x}{\pred}{\cstr'}$ s.t. $\kvar \not \in \params{p}$.
%
\begin{alignat}{3}
\bcoz{By definition}
  && \osoln{\cstr}{\kvar} & = \ssoln{\cstr'}{\kvar} \notag \\
\bcoz{By Theorem~\ref{lem:defns}}
  && \osoln{\cstr}{\kvar} & \models \defns{\cstr'}{\kvar} \notag \\
\bcoz{By definition of validity}
  && \osoln{\cstr}{\kvar} & \models \csimpss{x}{\pred}{ (\defns{\cstr'}{\kvar}) } \notag \\
\bcoz{By Lemma~\ref{lem:flat-defn}}
  && \osoln{\cstr}{\kvar} & \models \defns{(\csimpss{x}{\pred}{\cstr'})}{\kvar} \notag \\
\bcoz{By the definition of $\scoped{\kvar}{\cstr}$ and Lemma~\ref{lem:scoped-definitions}}
  && \osoln{\cstr}{\kvar} & \models \defns{\cstr}{\kvar} \notag
\end{alignat}
\end{proof}

\vspace{-0.45in}

\begin{proof} (Theorem~\ref{thm:strongest})
By Theorem~\ref{thm:defns} it suffices to prove that
if   $\satisfies{\soln}{\cstr}$
then $\satisfies{\comp{\soln}{\osoln{\cstr}{\kvar}}}{\uses{\cstr}{\kvar}}$.
\begin{alignat}{3}
\bcoz{Let}
  && \scoped{\kvar}{\cstr} & \doteq \csimpss{y}{q}{\cstr'}
     \mbox{s.t. $\kvar \not \in \params{q}$ and $\osoln{\cstr}{\kvar} = \ssoln{\cstr'}{\kvar}$}
     \label{eq:def-scoped-1}\\
\bcoz{Assume}
  && \soln & \models \cstr \label{eq:use-sat-assm} \\
\bcoz{By (\ref{eq:def-scoped-1}),  Lemma~\ref{lem:scoped-sat}}
  && \soln & \models \csimpss{y}{q}{\cstr'} \label{eq:sol-models-cstr-prime} \\
\bcoz{By Lemma~\ref{lem:scoped-uses}, (\ref{eq:def-scoped-1})}
  && \uses{\cstr}{\kvar} & = \csimpss{y}{q}{(\uses{\cstr'}{\kvar})} \cup C \quad \mbox{where $\kvar \not \in C$}  \label{eq:use-sat-cases} \\ % \mbox{\BLC{is there an implicit use of a "FLATTEN-USES" rule here? ANS:YES}}
\bcoz{Hence, by (\ref{eq:scoped-use-a}) and (\ref{eq:scoped-use-b})}
  && \comp{\soln}{\osoln{\cstr}{\kvar}} & \models \uses{\cstr}{\kvar} \notag \\
%
\intertext{\quad \emph{Case: \quad $\satisfies{\comp{\soln}{\osoln{\cstr}{\kvar}}}{\csimpss{y}{q}{(\uses{\cstr'}{\kvar})}}$} (\ref{eq:scoped-use-a})}
\bcoz{By (\ref{eq:use-sat-assm},\ref{eq:use-sat-cases}), Lemma~\ref{lem:partition}}
  && \soln & \models  \csimpss{y}{q}{(\uses{\cstr'}{\kvar})} \label{eq:asm-case-b} \\
\bcoz{Let $\cstr'' \in \uses{\cstr'}{\kvar}$ s.t.}
  && \cstr'' & \equiv \csimpss{x_i}{\pred_i}{\pred} \mbox{ and $\kvar \not \in \pred$} \label{eq:asm-cstr-def} \\
\bcoz{By (\ref{eq:asm-case-b})}
  && \soln & \models \csimpss{y}{q}{\csimpss{x_i}{\pred_i}{\pred}} \notag \\
\bcoz{By \rulename{Sat-Ext}}
  && \soln, \binds{y}{q} & \models \csimpss{x_i}{\pred_i}{\pred} \notag \\
\bcoz{By (\ref{eq:sol-models-cstr-prime})}
  && \soln,\binds{y}{q} & \models \cstr' \notag \\
\bcoz{By (\ref{eq:def-scoped-1}), Lemma~\ref{lem:strong}, for $i=1 \ldots n$}
  && \soln,\binds{y}{q} & \models \apply{\ssoln{\cstr'}{\kvar}}{\pred_i} \Rightarrow \pred_i \notag \\
\bcoz{As $\osoln{\cstr}{\kvar} = \ssoln{\cstr'}{\kvar}$  (\ref{eq:def-scoped-1})}
  && \soln,\binds{y}{q} & \models \apply{\osoln{\cstr}{\kvar}}{\pred_i} \Rightarrow \pred_i \notag \\ % \mbox{\BLC{Lemma 5.7 only talks about the non-hat version? ANS: thats ok, see step}} \notag \\
\bcoz{By repeating Lemma~\ref{lem:strengthening} and $\kvar \not \in \pred$}
  && \soln,\binds{y}{q} & \models \apply{\osoln{\cstr}{\kvar}}{\csimpss{x_i}{\pred_i}{\pred}}  \notag \\
\bcoz{That is}
  && \soln,\binds{y}{q} & \models \apply{\osoln{\cstr}{\kvar}}{\cstr''} \notag \\
\bcoz{As by (\ref{eq:def-scoped-1}) $\kvar \not \in \params{q}$}
  && \soln & \models \apply{\osoln{\cstr}{\kvar}}{  \csimpss{y}{q}{\cstr''}} \notag \\
\bcoz{Thus, by (\ref{eq:asm-cstr-def})}
  && \soln & \models \apply{\osoln{\cstr}{\kvar}}{  \csimpss{y}{q}{\uses{\cstr'}{\kvar}}} \notag \\
\bcoz{And by Lemma~\ref{lem:valid-composition}}
  && \comp{\soln}{\osoln{\cstr}{\kvar}} & \models \csimpss{y}{q}{\uses{\cstr'}{\kvar}} \label{eq:scoped-use-a} \\
%
\intertext{\quad \emph{Case: \quad $\satisfies{\comp{\soln}{\osoln{\cstr}{\kvar}}}{C}$} (\ref{eq:scoped-use-b})}
\bcoz{By (\ref{eq:use-sat-assm}, \ref{eq:use-sat-cases}), Lemma~\ref{lem:partition}}
  && \soln & \models C \label{eq:soln-sat-c} \\
\bcoz{As $\kvar \not \in C$, $\domain{\osoln{\cstr}{\kvar}} = \{ \kvar \}$}
  && \apply{\osoln{\cstr}{\kvar}}{C} & = C \notag \\
\bcoz{By (\ref{eq:soln-sat-c})}
  && \soln & \models \apply{\osoln{\cstr}{\kvar}}{C} \notag \\
\bcoz{By Lemma~\ref{lem:valid-composition}}
  && \comp{\soln}{\osoln{\cstr}{\kvar}} & \models C \label{eq:scoped-use-b}
\end{alignat}
\end{proof}

\begin{lemma}[\textbf{Eliminate-Definitions}]\label{lem:elim-defs} % C
  $\flatten{\elimk{\kvar}{\cstr}} = \apply{\osoln{\cstr}{\kvar}}{\uses{\cstr}{\kvar}}$.
\end{lemma}

\begin{proof} (Lemma~\ref{lem:elim-defs})
%
The above follows from the observations that:
%
(a)~$\domain{\osoln{\cstr}{\kvar}} = \{ \kvar \}$,
%
(b)~$\elimk{\kvar}{\cstr} = \elimsol{\osoln{\cstr}{\kvar}}{\cstr}$, and
%
(c)~Lemma~\ref{lem:subst}, as $\domain{\osoln{\cstr}{\kvar}} = \{ \kvar \}$.
%
\end{proof}


\begin{proof} (Theorem~\ref{thm:elim})
%
Let $\cstr' = \elimk{\kvar}{\cstr} = \elimsol{\osoln{\cstr}{\kvar}}{\cstr}$.
We prove the two directions separately.

\smallskip

\emph{Case: $\cstr'$ is satisfiable implies $\cstr$ is satisfiable}
%
\begin{alignat}{3}
\bcoz{Assume $\cstr'$ is satisfiable with}
&& {\soln'} & \models {\cstr'} \notag \\
\bcoz{(by Lemma~\ref{lem:flatten})}
&& {\soln'} &  \models {\flatten{\cstr'}} \notag \\
\bcoz{(by Lemma~\ref{lem:elim-defs})}
&& {\soln'} &  \models {\apply{\osoln{\cstr}{\kvar}}{\uses{\cstr}{\kvar}}} \notag \\
\bcoz{(by Lemma~\ref{lem:valid-composition})}
&& {\comp{\soln'}{\osoln{\cstr}{\kvar}}} &  \models {\uses{\cstr}{\kvar}} \label{eq:sat-up} \\
\bcoz{(by Theorem~\ref{thm:defns}, Lemma~\ref{lem:sat-composition})}
&& {\comp{\soln'}{\osoln{\cstr}{\kvar}}} & \models {\defns{\cstr}{\kvar}} \label{eq:sat-dn} \\
\bcoz{By~\ref{eq:sat-up},~\ref{eq:sat-dn}, Lemma~\ref{lem:partition}}
&& {\comp{\soln'}{\osoln{\cstr}{\kvar}}} & \models \cstr   \quad \mbox{\ie~$\cstr$ is satisfiable.} \notag \\
%
\intertext{\quad \emph{Case: $\cstr$ is satisfiable implies $\cstr'$ is satisfiable}}
%
\bcoz{Assume $\cstr$ is satisfiable with}
&& {\soln} & \models {\cstr} \notag \\
\bcoz{by Theorem~\ref{thm:strongest}}
&& \comp{\soln}{\osoln{\cstr}{\kvar}} & \models \cstr  \notag \\
\bcoz{by Lemma~\ref{lem:partition}}
&& \comp{\soln}{\osoln{\cstr}{\kvar}} & \models \uses{\cstr}{\kvar}  \notag \\
\bcoz{by Lemma~\ref{lem:valid-composition}}
&& \soln & \models \apply{\osoln{\cstr}{\kvar}}{\uses{\cstr}{\kvar}}  \notag \\
\bcoz{by Lemma~\ref{lem:elim-defs}}
&& \soln & \models \flatten{\cstr'} \quad \mbox{\ie by Lemma~\ref{lem:flatten} $\cstr'$ is satisfiable.} \notag
\end{alignat}
\end{proof}


==> 09-state.tex <==
\section{Appendix: Example}
\label{sec:example}

$\texttt{tick}$ is a stateful computation that updates an integer state by one and returns the old state. The standard state monad is lifted to the Hoare state monad that takes a pair of predicates which must hold on the initial and final worlds of the computation. We augment the Hoare monad's operations with implicit parameters to automatically track the state of the ``world'' as it flows through stateful computations. The type checker can then leverage refinement implicits to intrinsically prove the correctness of $\texttt{tick}$. The code is shown below.

\begin{code}
type W x = \s -> s = w

(>>=) :: w1:s ~> w2:s ~> w3:s ~>
  ST<W w1, W w2> s a ->
  (a -> ST<W w2, W w3> s b) -> 
  ST<W w1, W w3> s b

(>>) :: w1:s ~> w2:s ~> w3:s ~>
  ST<W w1, W w2> s a ->
  ST<W w2, W w3> s b -> 
  ST<W w1, W w3> s b

return :: w ~> ST<W w, W w> s a
  
get :: val ~> ST<W val, W val> s {v:s | v = val}
get = ST (\s -> (s, s))

put :: new:s -> ST<True, W new> s ()
put new = ST (\_ -> ((), new))

tick :: n ~> ST<W n, W (n+1)> Int {v:Int | v = n}
tick = do
  n <- get
  put (n + 1)
  return n
\end{code}

The elaborated code and ANF'd body of tick are shown below.

\begin{code}
tick =
  let f = (\n ->
    let rn = (let w1 = ? in @return w1 n) in
    let np = n + 1 in
    let pn = put np in
    let w2 = ? in let w3 = ? in let w4 = ? in
      @(>>) w2 w3 w4 pn rn) in

  let ge = (let w8 = ? in @get w8) in
  let w5 = ? in let w6 = ? in let w7 = ? in
    @(>>=) ge f
\end{code}

This generates the following subtyping constraints:

\begin{flalign*}
& \fbd{n}{\tint}, \ebd{w_1}{\tint} \vdash\\
& \qquad \ST{\lambda v. w_1 = v}{\lambda v. w_1 = v}{\reftnoty{v}{v = n}} \preceq \ST{\lambda v.\kappa_1(v)}{\lambda v.\kappa_2(v)}{\reftnoty{v}{\kappa_2(v)}}\\
& \fbd{n}{\tint} \vdash\\
& \qquad \reftnoty{v}{v = n + 1} \preceq \reftnoty{v}{\kappa_{np}(v)}\\
& \fbd{n}{\tint}, \fbd{np}{\reftpv{np}{\tint}{\kappa_{np}(np)}} \vdash\\
& \qquad \ST{\lambda v.\top}{\lambda v. np = v}{1} \preceq \ST{\lambda v.\kappa_4(v)}{\lambda v. \kappa_5(v)}{\reftnoty{v}{\kappa_6(v)}}\\
& \fbd{n}{\tint}, \fbd{np}{\reftpv{np}{\tint}{\kappa_{np}(np)}}, \ebd{w_2}{\tint}, \ebd{w_3}{\tint}, \ebd{w_4}{\tint} \vdash\\
& \qquad \ST{\lambda v.\kappa_1(v)}{\lambda v.\kappa_2(v)}{\reftnoty{v}{\kappa_3(v)}} \preceq \ST{\lambda v. w_3 = v}{\lambda v. w_4 = v}{\tint}\\
& \fbd{n}{\tint}, \fbd{np}{\reftpv{np}{\tint}{\kappa_{np}(np)}}, \ebd{w_2}{\tint}, \ebd{w_3}{\tint}, \ebd{w_4}{\tint} \vdash\\
& \qquad \ST{\lambda v.\kappa_4(v)}{\lambda v.\kappa_5(v)}{\reftnoty{v}{\kappa_6(v)}} \preceq \ST{\lambda v. w_2 = v}{\lambda v. w_3 = v}{1}\\
& \fbd{n}{\tint}, \fbd{np}{\reftpv{np}{\tint}{\kappa_{np}(np)}}, \ebd{w_2}{\tint}, \ebd{w_3}{\tint}, \ebd{w_4}{\tint} \vdash\\
& \qquad \ST{\lambda v. w_2 = v}{\lambda v. w_4 = v}{\tint} \preceq \ST{\lambda v.\kappa_7(v)}{\lambda v.\kappa_8(v)}{\reftnoty{v}{\kappa_9(v)}}\\
& \ebd{w8}{\tint} \vdash\\
& \qquad \ST{\lambda v. w_8 = v}{\lambda v. w_8 = v}{\reftnoty{v}{w_8 = v}} \preceq \ST{\lambda v.\kappa_{10}(v)}{\lambda v.\kappa_{11}(v)}{\reftnoty{v}{\kappa_{12}(v)}}\\
& \ebd{w_8}{\tint}, \ebd{w_5}{\tint}, \ebd{w_6}{\tint}, \ebd{w_7}{\tint} \vdash\\
& \qquad \ST{\lambda v.\kappa_{10}(v)}{\lambda v.\kappa_{11}(v)}{\reftnoty{v}{\kappa_{12}(v)}} \preceq \ST{\lambda v. w_5 = v}{\lambda v. w_6 = v}{\reftnoty{v}{\kappa_{13}(v)}}\\
& \ebd{w_8}{\tint}, \ebd{w_5}{\tint}, \ebd{w_6}{\tint}, \ebd{w_7}{\tint} \vdash\\
& \qquad \ST{\lambda v.\kappa_{7}(v)}{\lambda v.\kappa_{8}(v)}{\reftnoty{v}{\kappa_{9}(v)}} \preceq \ST{\lambda v. w_6 = v}{\lambda v. w_7 = v}{\reftnoty{v}{\kappa_{14}(v)}}\\
& \ebd{w_8}{\tint}, \ebd{w_5}{\tint}, \ebd{w_6}{\tint}, \ebd{w_7}{\tint} \vdash\\
& \qquad \ST{\lambda v. w_5 = v}{\lambda v. w_6 = v}{\reftnoty{v}{\kappa_{14}(v)}} \preceq \ST{\lambda v.\kappa_{15}(v)}{\lambda v.\kappa_{16}(v)}{\reftnoty{v}{\kappa_{17}(v)}}\\
& \fbd{n}{\tint} \vdash\\
& \qquad \ST{\lambda v.\kappa_{15}(v)}{\lambda v.\kappa_{16}(v)}{\reftnoty{v}{\kappa_{17}(v)}} \preceq \ST{\lambda v. n = v}{w (n + 1)}{\reftnoty{v}{v = n}}\\
\end{flalign*}

Which generates the following Existential Horn Clause:

$$\begin{array}{llll}
\forall n.\\
& \exists w_1.\\
& & \forall v. k_1(v) &\Rightarrow v = w_1\\
& & \forall v. v = w_1 &\Rightarrow k_2(v)\\
& & \forall v. v = n &\Rightarrow k_{3 }(v)\\
& \forall v. v = n+1 &\Rightarrow k_{np}(v)\\
& \forall np. k_{np}(np) &\Rightarrow\\
& & \forall v. k_4(v) &\Rightarrow true\\
& & \forall v. v=np &\Rightarrow k_5(v)\\
& & \forall v. v = () &\Rightarrow k_6(v)\\
& \exists w_2 . \exists w_3 . \exists w_4\\
& & \forall v. v=w_2 &\Rightarrow k_4(v)\\
& & \forall v. k_5(v) &\Rightarrow v=w_3\\
& & \forall v. k_6(v) &\Rightarrow v = ()\\
& & \forall v. v = w_3 &\Rightarrow k_1(v)\\
& & \forall v. k_2(v) &\Rightarrow v=w_4\\
& & \forall v. k_3(v) &\Rightarrow true\\
& & \forall v. k_7(v) &\Rightarrow v=w_2\\
& & \forall v. v=w_4 &\Rightarrow k_8(v)\\
& & \forall v. true &\Rightarrow k_9(v)\\
& \exists w_8.\\
& & \forall v. k_{10}(v) &\Rightarrow v=w_8\\
& & \forall v. v=w_8 &\Rightarrow k_{11}(v)\\
& & \forall v. v=w_8 &\Rightarrow k_{12}(v)\\
& \exists w_5. \exists w_6. \exists w_7\\
& & \forall v. v=w_5 &\Rightarrow k_{10}(v)\\
& & \forall v. k_{11}(v) &\Rightarrow v=w_6\\
& & \forall v. k_{12}(v) &\Rightarrow k_{13}(v)\\
& & \forall v. v=w_6 &\Rightarrow k_7(v)\\
& & \forall v. k_8(v) &\Rightarrow v=w_7\\
& & \forall v. k_9(v) &\Rightarrow k_{14}(v)\\
& & \forall v. k_{15}(v) &\Rightarrow v=w_5\\
& & \forall v. v=w_6 &\Rightarrow k_{16}(v)\\
& & \forall v. k_{14}(v) &\Rightarrow k_{17}(v)\\
\forall v. v=n &\Rightarrow k_{15}(v)\\
\forall v. k_{16}(v) &\Rightarrow v=n+1\\
\forall v. k_{17}(v) &\Rightarrow v=n\\
\end{array}$$


==> Makefile <==
all: pdf

pdf:
	latexmk -pdf main.tex

cont: continuous
continuous:
	latexmk -pvc -pdf -interaction=nonstopmode main.tex

chop:
	rm -f anon-supplemental.pdf anon-submission.pdf
	cp main.pdf anon-supplemental.pdf
	if which cpdf; \
         then cpdf  anon-supplemental.pdf "1-28" -o anon-submission.pdf; \
         else pdftk anon-supplemental.pdf cat 1-28 output anon-submission.pdf; fi

plain:
	touch no-editing-marks
	$(MAKE) clean
	$(MAKE) 

ed:
	rm -f no-editing-marks
	$(MAKE) clean
	$(MAKE)

clean:
	latexmk -c main.tex

cleanall:
	latexmk -C -bibtex main.tex

.PHONY: all pdf clean cleanall cont continuous plain ed


==> acknowledgements.tex <==
Tristan
Shravan
MJ
Alex
Peter
Dylan for food

==> rscListings.tex <==
\definecolor{haskellblue}{rgb}{0.0, 0.0, 1.0}
\definecolor{haskellblue}{rgb}{1.0, 0.0, 0.0}
\definecolor{gray_ulisses}{gray}{0.55}
\definecolor{castanho_ulisses}{rgb}{0.71,0.33,0.14}
\definecolor{preto_ulisses}{rgb}{0.41,0.20,0.04}
\definecolor{green_ulisses}{rgb}{0.0,0.4,0.0}
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}
\definecolor{darkgray}{gray}{0.30}
\definecolor{darkblue}{rgb}{0,0,0.75}
\definecolor{darkgreen}{rgb}{0,0.4,0}

\lstdefinelanguage{RefScript}{
  basicstyle=\ttfamily\footnotesize,
  backgroundcolor=\color{white},  
  sensitive=true,
  keywords={typeof, instanceof, new, true, false, catch, function, return, 
            null, catch, switch, var, if, in, for, while, do, 
            else, case, break, forall, type, true, false,  
            constructor, super, public, private, class, 
            interface, extends, implements, module, 
            declare, this,let, then, undefined, fn,
            },
  keywordstyle=\color{mymauve},
  morecomment=[s]{/*}{*/},
  morecomment=[l]//,
  morestring=[b]",
  morestring=[b]',
  commentstyle=\color{mygreen},
  stringstyle=\color{darkgreen},
  showstringspaces=false,
  numberblanklines=true,
  showspaces=false,
  breaklines=true,
  showtabs=false,
  emph={[1] reduce, $reduce,minIndexFO,minIndexHO, minIndex, neg,
            neg\#1, neg\#2, step},
  emphstyle={[1]\color{darkblue}},
  emph={[2]     boolean, bool,tt,ff,any,void,number,string,nat,index,idx,Array},
  emphstyle={[2]\color{darkgreen}},
  literate= {=>}{$\Rightarrow$}{1}
            {>=}{{$\geq$}}1
            {<=}{{$\leq$}}1
            {\/\\}{{$\wedge$}}2
}

\lstnewenvironment{code}{\lstset{language=RefScript}}{}

\lstMakeShortInline[language=RefScript, basicstyle=\normalsize\ttfamily]@



==> scratch.tex <==
asd

\begin{figure}[t]
\begin{subfigure}[h]{0.49\textwidth}
\begin{code}
tick :: n:Int ~> SST n (n+1) Int n 
tick = do
  n <- get
  put (n + 1)
  return n
\end{code}
\caption{Incrementing an Integer State}
\label{tick}
\end{subfigure}
\begin{subfigure}[h]{0.499\textwidth}
  \scriptsize
\begin{code}
data ST p q s a 
  = ST (s -> (s, a))
-- Singleton ST
type SST i o s a 
  = ST {v:s|v=i} {v:s|v=o} s a 

-- Monadic Interface
(>>=)  :: w1:s ~> w2:s ~> w3:s ~> 
          SST w1 w2 s a -> 
          (a -> SST w2 w3 s b) -> 
          SST w1 w3 s b

return :: w ~> a -> SST w w s a 

-- read and write the state
get :: w ~> SST w w s w 
get = ST (\s -> (s, s))

put :: w:s -> ST s {v:s|v=w} s ()
put w = ST (\_ -> ((), w))
\end{code}
\caption{Monadic Interface to the Hoare State Monad}
\label{statemonad}
\end{subfigure}
\caption{Verifying a Stateful Computation}
\label{stateex}
\vspace{-4ex}
\end{figure}
\MK{Something is missing on ST}

